SPATL: Salient Parameter Aggregation and Transfer Learning for Heterogeneous Clients in Federated Learning

Federated learning~(FL) facilitates the training and deploying AI models on edge devices. Preserving user data privacy in FL introduces several challenges, including expensive communication costs, limited resources, and data heterogeneity. In this paper, we propose SPATL, an FL method that addresses these issues by: (a) introducing a salient parameter selection agent and communicating selected parameters only; (b) splitting a model into a shared encoder and a local predictor, and transferring its knowledge to heterogeneous clients via the locally customized predictor. Additionally, we leverage a gradient control mechanism to further speed up model convergence and increase robustness of training processes. Experiments demonstrate that SPATL reduces communication overhead, accelerates model inference, and enables stable training processes with better results compared to state-of-the-art methods. Our approach reduces communication cost by up to $86.45\%$, accelerates local inference by reducing up to $39.7\%$ FLOPs on VGG-11, and requires $7.4 \times$ less communication overhead when training ResNet-20.

==> content/06_limitation.tex <==
\subsection{Limitations}
\label{sec:lim}
The proposed approach may have poor performance on simple models. As Figure~\ref{fig:vgg_cifar} shows, our approach works well on over-parameterized neural networks, such as ResNet~\cite{he2016resnet} and VGG~\cite{simonyan2015vgg} net. However, when it turns to a less-parameterized model, such as 2-layer CNN, the salient parameter selection may degrade its performance, making the model converge slower than the baselines. Generally, the less-parameterized models are rarely being used in real-world applications.

%Additionally, we only test our approach on a federated learning setting of 10 clients with a sample ratio=1.

==> figure/f_gradient_control.tex <==
\begin{figure}
 \begin{center}

\centerline{\includegraphics[width=.8\columnwidth]{figure/gradient_control.pdf}}
\caption{Gradient control vs. no gradient control.}
 \vskip -0.4in
\label{fig:grad_control}
\end{center}
 \end{figure}

==> figure/f_transfer_ablation.tex <==

 
 \begin{figure}
 \begin{center}

\centerline{\includegraphics[width=.8\columnwidth]{figure/transfer.pdf}}
\caption{Gradient control vs. no gradient control.}
 \vskip -0.4in
\label{fig:grad_control}
\end{center}
 \end{figure}

==> figure/fsub_select_aggregate.tex <==
% \begin{figure}
% \centering
% \begin{subfigure}

%     \centerline{\includegraphics[width=0.4\linewidth]{figure/pram_slect_agent.pdf}}
%     \caption{Parameter selection with reinforcement learning. The parameter selection agent selects a salient parameter and uses the selected sub-model's accuracy to search for the desired policy.}
    
%     \label{fig:pram_selction}
% \end{subfigure}%
% \begin{subfigure}
%  \begin{center}

% \centerline{\includegraphics[width=.4\linewidth]{figure/aggregate.pdf}}
% \caption{Aggregation with salient parameter. For each client, the aggregator will aggregate partial parameters corresponding to the client's salient parameter. }

% \label{fig:pram_aggre}
% \end{center}

% \end{subfigure}
% \caption{A figure with two subfigures}
% \label{fig:test}
% \end{figure}

\begin{figure}%
    \centering
    \subfloat[\centering Parameter selection. ]{{\includegraphics[width=.5\linewidth]{figure/pram_slect_agent.pdf} }}%
    \qquad
    \subfloat[\centering Salient parameter aggregation]{{\includegraphics[width=.3\linewidth]{figure/aggregate.pdf} }}%
    \caption{(a) The parameter selection agent selects a salient parameter and uses the selected sub-model's accuracy to search for the desired policy. (b). For each client, the aggregator will aggregate partial parameters corresponding to the client's salient parameter.}%
    \label{fig:param_selection}%
\end{figure}

==> table/t_com_cost.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
  \caption{Communication cost.}
  \label{tab:com_cost}
 
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|ccc|c|ccc|c|ccc}
\hline
Method   & Model                  & R                 & Avg. cost/ (R*C) & Total               & Model                  & R                 & Avg. cost/(R*C) & Total               & Model                  & R                 & Avg. cost / (R*C) & Total              \\ \hline
FedAvg   & \multirow{5}{*}{Res20} & \textgreater{}200 & 2.1MB            & \textgreater{}4.2GB & \multirow{5}{*}{Res32} & \textgreater{}200 & 3.2MB           & \textgreater{}6.4GB & \multirow{5}{*}{Vgg11} & 181               & 42MB              & 76GB               \\
FedNova  &                        & 198               & 4.2MB            & 8.32GB              &                        & 197               & 6.4MB           & 12.6GB              &                        & 159               & 84MB              & 136GB              \\
FedProx  &                        & \textgreater{}200 & 2.1MB            & \textgreater{}4.2GB &                        & \textgreater{}200 & 3.2MB           & \textgreater{}6.4GB &                        & \textgreater{}200 & 42 MB             & \textgreater{}84GB \\
SCAFFOLD &                        & 49                & 4.3MB            & 2.1GB               &                        & 55                & 6.5MB           & 3.6GB               &                        & 54                & 84 MB             & 45GB               \\
SPATL    &                        & 52                & 2.1MB            & 1.1GB               &                        & 50                & 3.6MB           & 1.8GB               &                        & 46                & 61.3 MB           & 28GB               \\ \hline
\end{tabular}%
}
\end{table*}

==> table/t_com_cost_converge.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}
  \caption{Communication cost of SoTAs to converge.}
  \label{tab:com_cost2}
\centering
{%
\begin{tabular}{lccccc}
\hline
Method         & Model                   & Clients             & Acc $\%$       &  Cost/ (R*C) & Total            \\ \hline
FedAvg         & \multirow{5}{*}{Res20}  & \multirow{5}{*}{30} & 60.58          & 2.1MB  & 12.42GB          \\
FedNova        &                         &                     & 64.50          & 4.2MB  & 24.12GB          \\
FedProx        &                         &                     & 60.20          & 2.1MB  & 12.43GB          \\
SCAFFOLD       &                         &                     & 10.00          & 4.3MB  & diverge          \\
SPATL          &                         &                     & 66.49          & 2.1MB  & 11.99GB          \\ \hline
FedAvg         & \multirow{5}{*}{Res32}  & \multirow{5}{*}{30} & 64.92          & 3.2MB  & 18.94GB          \\
FedNova        &                         &                     & 67.48          & 6.4MB  & 37.69GB          \\
FedProx        &                         &                     & 64.75          & 3.2MB  & 18.75GB          \\
SCAFFOLD       &                         &                     & 10.00          & 6.5MB  & diverge          \\
SPATL          &                         &                     & 70.23          & 3.6MB  & 20.78GB          \\ \hline
FedAvg         & \multirow{5}{*}{VGG-11} & \multirow{5}{*}{50} & 32.68          & 42MB   & 412GB            \\
FedNova        &                         &                     & 29.90          & 84MB   & 824GB            \\
FedProx        &                         &                     & 32.14          & 42MB   & 414GB            \\
SCAFFOLD       &                         &                     & 10.00          & 84MB   & diverge          \\
SPATL          &                         &                     & 49.76          & 61MB   & 586GB            \\ \hline
FedAvg         & \multirow{5}{*}{Res20}  & \multirow{5}{*}{50} & 32.71          & 2.1MB  & 20.71GB          \\
FedNova        &                         &                     & 29.08          & 4.2MB  & 38.35GB          \\
FedProx        &                         &                     & 32.43          & 2.1MB  & 20.20GB          \\
SCAFFOLD       &                         &                     & 10.00          & 4.3MB  & diverge          \\
{SPATL (Ours)} &                         &                     & {42.54} & 2.1MB  & {18.05GB}\\ \hline
\end{tabular}
}
\end{table}

==> table/t_com_vertical.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}
\centering
  \caption{Communication cost of SoTAs to achieves 80\% accuracy. }
  \label{tab:com_cost}
%  R stands for communication rounds, and Avg. cost/ (R*C) represents average communication cost of a single client in a round.
\resizebox{\linewidth}{!}{%
\begin{tabular}{ccccc}
\hline
Method   & Model                  & Rounds                 & Cost/ (R*C) & Total  \\ \hline
FedAvg$^+$   & \multirow{5}{*}{Res20} & \textgreater{}400 & 2.1MB            & 8.4GB  \\
FedNova  &                        & 198               & 4.2MB            & 8.32GB \\
FedProx$^+$  &                        & \textgreater{}400 & 2.1MB            & 8.4GB  \\
SCAFFOLD &                        & 49                & 4.3MB            & 2.1GB  \\
 \textbf{SPATL}    &                        & 52                & 2.1MB            &  \textbf{1.1GB}  \\ \hline
FedAvg$^+$   & \multirow{5}{*}{Res32} & \textgreater{}400 & 3.2MB            & 12.8GB  \\
FedNova  &                        & 197               & 6.4MB            & 12.6GB \\
FedProx$^+$  &                        & \textgreater{}400 & 3.2MB            & 12.8GB  \\
SCAFFOLD &                        & 55                & 6.5MB            & 3.6GB  \\
\textbf{SPATL}    &                        & \textbf{50}                & 3.6MB            & \textbf{1.8GB}  \\ \hline
FedAvg   & \multirow{5}{*}{VGG11}   & 181               & 42MB             & 76GB   \\
FedNova  &                        & 159               & 84MB             & 136GB  \\
FedProx$^+$  &                        & \textgreater{}400 & 42 MB            & 168GB   \\
SCAFFOLD &                        & 54                & 84 MB            & 45GB   \\
\textbf{SPATL}    &                        & \textbf{46}                & 61.3 MB          & \textbf{28GB}   \\ \hline
\end{tabular}%
}
\end{table}
